Unsupervised Learning for Class Distribution Mismatch

Class distribution mismatch (CDM) refers to the discrepancy between class distributions in training data and target tasks. Previous methods address this by designing classifiers to categorize classes known during training, while grouping unknown or new classes into an "other" category. However, they focus on semi-supervised scenarios and heavily rely on labeled data, limiting their applicability and performance. To address this, we propose Unsupervised Learning for Class Distribution Mismatch (UCDM), which constructs positive-negative pairs from unlabeled data for classifier training. Our approach randomly samples images and uses a diffusion model to add or erase semantic classes, synthesizing diverse training pairs. Additionally, we introduce a confidence-based labeling mechanism that iteratively assigns pseudo-labels to valuable real-world data and incorporates them into the training process. Extensive experiments on three datasets demonstrate UCDM's superiority over previous semi-supervised methods. Specifically, with a 60% mismatch proportion on Tiny-ImageNet dataset, our approach, without relying on labeled data, surpasses OpenMatch (with 40 labels per class) by 35.1%, 63.7%, and 72.5% in classifying known, unknown, and new classes.

==> content/diffusion.tex <==
\section{Related Work}

\subsection{Diffusion Probabilistic Models}

Diffusion probabilistic models (DPMs) are a class of generative models consisting of a forward diffusion process and a reverse denoising process. The forward process is a Markov chain that gradually adds noise to the data via a Gaussian transition, defined as \( q(\bm{x}_{t} \mid \bm{x}_{t-1}) = \mathcal{N}(\sqrt{1 - \beta_t}\bm{x}_{t-1}, \beta_t\bm{I}) \), where \( \{\beta_t\}_{t=0}^T \) represents a fixed or learned variance schedule. This process produces a latent variable \( \bm{x}_t \), which can be formalized as~\myref{forward}. 
\begin{equation}\label{forward}
    \bm{x}_t = \sqrt{\alpha_t}\bm{x}_0 + \sqrt{1 - \alpha_t} \bm{\epsilon}, \quad \bm{\epsilon} \sim \mathcal{N}(0,1)
\end{equation}
where \( \bm{x}_0 \sim q(\bm{x}_0) \) and \( \alpha_t = \prod_{s=1}^t (1 - \beta_s) \).

In the reverse process, given a noise variable \( \bm{x}_t \), the model gradually removes the noise through a parameterized Gaussian transition \( p_{\theta}(\bm{x}_{t-1} \mid \bm{x}_t) = \mathcal{N}(\bm{x}_{t-1}; \mu_{\theta}(\bm{x}_t, t), \) \(\sigma_{\theta}(\bm{x}_t, t)\bm{I}) \), where \( \sigma_{\theta}(\bm{x}_t, t) \) are time-dependent constants that remain untrained. 
% This reverse diffusion effectively denoises the variable, enabling the generation of structured data.
To estimate \( \mu_{\theta}(\bm{x}_t, t) \), the text-guided diffusion probabilistic model, which aims to map a noise vector and a textual condition \( \mathcal{C} \) to an output image, trains a noise estimator \( \epsilon_{\theta}(\bm{x}_t, t, \mathcal{C}) \) by minimizing the~\myref{obj}. 
\begin{equation}\label{obj}
    \min\limits_{\bm{\theta}} \mathbb{E}_{\bm{x}_0 \sim q(\bm{x}_0), \bm{\epsilon} \sim \mathcal{N}(\bm{0}, \bm{I}), t} \|\bm{\epsilon} - \epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})\|_2^2 
\end{equation}
where 
% \( \mathcal{C} = \varphi(\mathcal{P}) \) represents the text embedding, \( \varphi(\cdot) \) is the text encoder, and 
\( \epsilon_{\theta}(\bm{x}_t, t, \mathcal{C}) \) predicts the noise present in \( \bm{x}_t \) to reconstruct \( \bm{x}_{t-1} \).


% To to estimate ${\mu}_{\theta}(\bm{x}_t, t)$, text-guided diffusion probabilistic model ,which aims to map a noise vector and textual condition $\mathcal{P}$ to an output image, trains a noise estimator $\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})$  by~\myref{obj}.
% \begin{equation}\label{obj}
%     \begin{aligned}
%         \min\limits_{\bm{\theta}} \mathbb{E}_{\bm{x}_0 \sim q(\bm{x}_0), \bm{\epsilon} \sim \mathcal{N}(\bm{0}, \bm{I}), t} \|\bm{\epsilon} - \epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})\|_2^2 
%     \end{aligned}
% \end{equation} 
% where $\mathcal{C} = \varphi(\mathcal{P})$ is the text embedding,  $\varphi(\cdot)$ is a text encoder, and $\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})$ predicts the noise in $\bm{x}_t$ to reconstruct $\bm{x}_{t-1}$.

% After training $\epsilon_{\theta}(\bm{x}_t,t, \mathcal{C})$, in denoising diffusion implicit models (DDIM), the new data is generated by iteratively apply the update rule ~\myref{ddim} until step 0.
% \begin{equation}\label{ddim2}
%     \begin{aligned}
%         {\bm{x}_{t-1}} = \sqrt{\frac{\alpha_{t-1}}{\alpha_t}}\bm{x}_t - \sqrt{\alpha_{t-1}}\psi(\alpha_t, \alpha_{t-1})\hat\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})
%     \end{aligned}
% \end{equation} 
% where $\hat\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})=\epsilon_{\theta}(\bm{x}_t, t, \emptyset) + \gamma \left[\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})-\epsilon_{\theta}(\bm{x}_t, \right.\\ \left. t, \emptyset )\right]$.
% $\epsilon_{\theta}(\bm{x}_t, t, \emptyset)$ is a unconditional DPM with null-text $\emptyset=\varphi(\text{``''})$, and $\gamma$ is a parameter that controls the strength of text guidance. We simplify the notation $\epsilon_{\theta}(\bm{x}_t, t, \emptyset)$ with $\epsilon_{\theta}(\bm{x}_t, t)$ in following. 




% After training \( \epsilon_{\theta}(\bm{x}_t, t, \mathcal{C}) \), the new data is generated by iteratively applying the update rule in~\myref{ddim2} until reaching step 0. 
% \begin{equation}\label{ddim2}
%     \bm{x}_{t-1} \!\!= \!\!\sqrt{\frac{\alpha_{t-1}}{\alpha_t}} \bm{x}_t \!-\! \sqrt{\alpha_{t-1}} \psi(\alpha_t, \alpha_{t-1}, \sigma_t) \hat{\epsilon}_{\theta}(\bm{x}_t, t, \mathcal{C}) + \sigma_t \epsilon_t
% \end{equation}
% where $\psi(\alpha_t, \alpha_{t-1}, \sigma_t) = \sqrt{\frac{1}{\alpha_t}-1}-\sqrt{\frac{1-\alpha_{t-1}-\sigma_t^2}{\alpha_{t-1}}}$ and $\hat\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})=\epsilon_{\theta}(\bm{x}_t, t, \emptyset) + \gamma \left[\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})-\epsilon_{\theta}(\bm{x}_t,  t, \emptyset )\right]$;  when $\sigma_t = 0$ for all $t$, the coefficient before the random
% noise $\epsilon_t$ becomes zero, and then the resulting model becomes an implicit probabilistic model, named  denoising diffusion implicit model(DDIM), where samples are generated from $\bm{x}_T$ to $\bm{x}_0$ with a fixed procedure. Here, \( \epsilon_{\theta}(\bm{x}_t, t, \emptyset) \) is the unconditional DPM, with null-text \( \emptyset = \varphi(\text{``''}) \), and \( \gamma \) is a parameter that controls the strength of the text guidance. For simplicity, we denote \( \epsilon_{\theta}(\bm{x}_t, t, \emptyset) \) as \( \epsilon_{\theta}(\bm{x}_t, t) \) in the following.


After training \( \epsilon_{\theta}(\bm{x}_t, t, \mathcal{C}) \), new data is generated by iteratively applying the update rule in~\myref{ddim2} until step 0 is reached:  
\begin{equation}\label{ddim2}
\bm{x}_{t-1} \!\!= \!\!\sqrt{\frac{\alpha_{t-1}}{\alpha_t}} \bm{x}_t - \sqrt{\alpha_{t-1}} \psi(\alpha_t, \alpha_{t-1}, \sigma_t) \hat{\epsilon}_{\theta}(\bm{x}_t, t, \mathcal{C}) + \sigma_t \epsilon_t
\end{equation}
where \( \psi(\alpha_t, \alpha_{t-1}, \sigma_t) = \sqrt{\frac{1}{\alpha_t}-1} - \sqrt{\frac{1-\alpha_{t-1}-\sigma_t^2}{\alpha_{t-1}}} \), and \( \hat{\epsilon}_{\theta}(\bm{x}_t, t, \mathcal{C}) = \epsilon_{\theta}(\bm{x}_t, t, \emptyset) + \gamma \left[\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C}) - \epsilon_{\theta}(\bm{x}_t, t, \emptyset)\right] \). When \( \sigma_t = 0 \) for all \( t \), the coefficient before the random noise \( \epsilon_t \) becomes zero, resulting in an implicit probabilistic model named the Denoising Diffusion Implicit Model (DDIM). This enables sample generation from \( \bm{x}_T \) to \( \bm{x}_0 \) through a fixed deterministic procedure.  Moreover, \( \epsilon_{\theta}(\bm{x}_t, t, \emptyset) \) is the unconditional DPM using null-text encoding \( \emptyset = \varphi(\text{``''}) \), and \( \gamma \) controls the strength of text guidance. For simplicity, \( \epsilon_{\theta}(\bm{x}_t, t, \emptyset) \) is denoted as \( \epsilon_{\theta}(\bm{x}_t, t) \) in the subsequent discussion.  













% After training \( \epsilon_{\theta}(\bm{x}_t, t, \mathcal{C}) \), the denoising diffusion implicit models (DDIM) generate new data by iteratively applying the update rule in~\myref{ddim2} until reaching step 0. 
% \begin{equation}\label{ddim2}
%     \bm{x}_{t-1} = \sqrt{\frac{\alpha_{t-1}}{\alpha_t}} \bm{x}_t - \sqrt{\alpha_{t-1}} \psi(\alpha_t, \alpha_{t-1}) \hat{\epsilon}_{\theta}(\bm{x}_t, t, \mathcal{C})
% \end{equation}
% where $\psi(\alpha_t, \alpha_{t-1}) = \sqrt{\frac{1}{\alpha_t}-1}-\sqrt{\frac{1}{\alpha_{t-1}}-1}$, and $\hat\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})=\epsilon_{\theta}(\bm{x}_t, t, \emptyset) + \gamma \left[\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})-\epsilon_{\theta}(\bm{x}_t, \right.\\ \left. t, \emptyset )\right]$. Here, \( \epsilon_{\theta}(\bm{x}_t, t, \emptyset) \) is the unconditional DPM, with null-text \( \emptyset = \varphi(\text{``''}) \), and \( \gamma \) is a parameter that controls the strength of the text guidance. For simplicity, we denote \( \epsilon_{\theta}(\bm{x}_t, t, \emptyset) \) as \( \epsilon_{\theta}(\bm{x}_t, t) \) in the following.









Furthermore, it has been established that this sampling process corresponds to  that of score-based generative models, with the relationships shown in~\myref{uncon_grdient} and~\myref{con_grdient}, respectively.
\begin{equation}\label{uncon_grdient}
    \epsilon_{\theta}(\bm{x}_t, t) = -\sqrt{1 - \bar{\alpha}_t} \nabla_{\bm{x}_t} \log p_{\theta}(\bm{x}_t)
\end{equation}
\begin{equation}\label{con_grdient}
    \epsilon_{\theta}(\bm{x}_t, t, \mathcal{C}) = -\sqrt{1 - \bar{\alpha}_t} \nabla_{\bm{x}_t} \log p_{\theta}(\bm{x}_t \mid \mathcal{C})
\end{equation}
where \( \bar{\alpha}_t = \prod_{i=0}^{t} \alpha_i \) and \( \nabla_{\bm{x}_t} \log p_{\theta}(\bm{x}_t) \) represents the gradient of the log-likelihood with respect to \( \bm{x}_t \), which indicates the direction in data space that maximizes its likelihood. Intuitively, since \( \epsilon_{\theta}(\bm{x}_t, t) \) predicts the noise added to \( \bm{x}_{t-1} \), moving in the opposite direction—i.e., denoising the image—represents the optimal update to increase the subsequent log-probability.


% Moreover, it was found that this sampling process corresponds to that of score-based generative models, with the relationships shown in~\myref{uncon_grdient} and~\myref{con_grdient}, respectively.
% \begin{equation}\label{uncon_grdient}
%     \begin{aligned}
%         \epsilon_{\theta}(\bm{x}_t,t) = -\sqrt{1 - \bar\alpha_t} \nabla \log p_{\theta}(\bm{x}_t)
%     \end{aligned}
% \end{equation}

% \begin{equation}\label{con_grdient}
%     \begin{aligned}
%         \epsilon_{\theta}(\bm{x}_t,t, \mathcal{C}) = -\sqrt{1 - \bar\alpha_t} \nabla \log p_{\theta}(\bm{x}_t | \mathcal{C})
%     \end{aligned}
% \end{equation}
% where ${\bar\alpha}_t = \prod_{i=0}^{t}\alpha_i$, and $\nabla \log p_{\theta}(\bm{x}_t)$ represents the gradient of the log-likelihood with respect to $\bm{x}_t$, essentially describing the direction in data space that would increase its likelihood. Intuitively, since $\epsilon_{\theta}(\bm{x}_t,t)$ predicts the noise added to $\bm{x}_t$, moving in its opposite direction (i.e., denoising the image) is the optimal update to increase the subsequent log probability.




% Moreover, it was found that this sampling process corresponds to that of score-based generative models with the relationship shown in~\myref{uncon_grdient} and ~\myref{con_grdient} respectively.
% \begin{equation}\label{uncon_grdient}
%     \begin{aligned}
%         \epsilon_{\theta}(\bm{x}_t,t)=-\sqrt{1-\bar\alpha_t} \nabla \log p_{\theta}(\bm{x}_t)
%     \end{aligned}
% \end{equation}
% \begin{equation}\label{con_grdient}
%     \begin{aligned}
%         \epsilon_{\theta}(\bm{x}_t,t, \mathcal{C})=-\sqrt{1-\bar\alpha_t} \nabla \log p_{\theta}(\bm{x}_t | \mathcal{C})
%     \end{aligned}
% \end{equation}
% where ${\bar\alpha}_t  = \prod_{i=0}^{t}\alpha_i$ and $\nabla \log p_{\theta}(\bm{x}_t)$ indicates the the gradients of log likelihood with respect to $\bm{x}_t$ essentially describes what direction in data space to move in order to further increase its likelihood. Intuitively, since the $\epsilon_{\theta}(\bm{x}_t,t)$ predicts the noise added to $\bm{x}_t$, moving in its opposite direction, i.e., denoises the image, would be the best update to increase the subsequent log probability. 

\subsection{Open-Set Learning}

% \newpage

% It was found that 
% \begin{equation}\label{con_grdient}
%     \begin{aligned}
%         \epsilon_{\theta}(\bm{x}_t,t, \mathcal{C})=-\sqrt{1-\bar\alpha_t} \nabla \log p_{\theta}(\bm{x}_t | \mathcal{C})
%     \end{aligned}
% \end{equation}

% The DDIM sampling process corresponding to $\epsilon_{\theta}(\bm{x}_t,t, \mathcal{C})$ is defined as
% \begin{equation}\label{ddim2}
%     \begin{aligned}
%         {\bm{x}_{t-1}} = \sqrt{\frac{\alpha_{t-1}}{\alpha_t}}\bm{x}_t - \sqrt{\alpha_{t-1}}\psi(\alpha_t, \alpha_{t-1})\hat\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})
%     \end{aligned}
% \end{equation} 
% where $\hat\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})=\epsilon_{\theta}(\bm{x}_t, t, \emptyset) + \gamma \left[\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})-\epsilon_{\theta}(\bm{x}_t, \right.\\ \left. t, \emptyset )\right]$.
% $\epsilon_{\theta}(\bm{x}_t, t, \emptyset)$ is a unconditional DPM with null-text $\emptyset=\varphi(\text{``''})$, and $\gamma$ is a parameter that controls the strength of text guidance.  It was found that this sampling process corresponds to that of score-based generative models with the relationship shown in~\myref{uncon_grdient} and ~\myref{con_grdient} respectively.
% \begin{equation}\label{uncon_grdient}
%     \begin{aligned}
%         &\epsilon_{\theta}(\bm{x}_t,t)=-\sqrt{1-\bar\alpha_t} \nabla \log p_{\theta}(\bm{x}_t)\\
%          \epsilon_{\theta}(\bm{x}_t,t, \mathcal{C})=-\sqrt{1-\bar\alpha_t} \nabla \log p_{\theta}(\bm{x}_t | \mathcal{C})
%     \end{aligned}
% \end{equation}
% % \begin{equation}\label{con_grdient}
% %     \begin{aligned}
% %         \epsilon_{\theta}(\bm{x}_t,t, \mathcal{C})=-\sqrt{1-\bar\alpha_t} \nabla \log p_{\theta}(\bm{x}_t | \mathcal{C})
% %     \end{aligned}
% % \end{equation}
% where ${\bar\alpha}_t  = \prod_{i=0}^{t}\alpha_i$ and $\nabla \log p_{\theta}(\bm{x}_t)$ indicates the the gradients of log likelihood with respect to $\bm{x}_t$ essentially describes what direction in data space to move in order to further increase its likelihood. Intuitively, since the $\epsilon_{\theta}(\bm{x}_t,t)$ predicts the noise added to $\bm{x}_t$, moving in its opposite direction, i.e., denoises the image, would be the best update to increase the subsequent log probability. 













% \textbf{Unconditional Diffusion Probabilistic Models.} To estimate ${\mu}_{\theta}(\bm{x}_t, t)$, a neural network $\epsilon_{\theta}(\bm{x}_t, t)$ is trained by~\myref{obj}.
% \begin{equation}\label{obj}
%     \begin{aligned}
%         \min\limits_{\bm{\theta}} \mathbb{E}_{\bm{x}_0 \sim q(\bm{x}_0), \bm{\epsilon} \sim \mathcal{N}(\bm{0}, \bm{I}), t} \|\bm{\epsilon} - \epsilon_{\theta}(\bm{x}_t, t)\|_2^2 
%     \end{aligned}
% \end{equation}

% % After training $\epsilon_{\theta}(\bm{x}_t, t)$, the data is sampled using~\myref{ddpm}.
% % \begin{equation}\label{ddpm}
% %     \begin{aligned}
% %         \bm{x}_{t-1]} = \sqrt{\frac{\alpha_{t-1}}{\alpha_t}}\left(\bm{x}_t, - \frac{\beta_t}{\sqrt{1-\alpha_t}}\epsilon_{\theta}(\bm{x}_t, t)\right) + 
% %     \end{aligned}
% % \end{equation}

% After training $\epsilon_{\theta}(\bm{x}_t, t)$, in denoising diffusion implicit models (DDIM), the new data is generated by iteratively apply the update rule ~\myref{ddim} until step 0.
% \begin{equation}\label{ddim}
%     \begin{aligned}
%         {\bm{x}_{t-1}} = \sqrt{\frac{\alpha_{t-1}}{\alpha_t}}\bm{x}_t - \sqrt{\alpha_{t-1}}\psi(\alpha_t, \alpha_{t-1})\epsilon_{\theta}(\bm{x}_t, t)
%     \end{aligned}
% \end{equation}
% where $\psi(\alpha_t, \alpha_{t-1}) = \sqrt{\frac{1}{\alpha_t}-1}-\sqrt{\frac{1}{\alpha_{t-1}}-1}$. Moreover, it was found that this sampling process corresponds to that of score-based generative models with the relationship shown in~\myref{uncon_grdient}.
% \begin{equation}\label{uncon_grdient}
%     \begin{aligned}
%         \epsilon_{\theta}(\bm{x}_t,t)=-\sqrt{1-\bar\alpha_t} \nabla \log p_{\theta}(\bm{x}_t)
%     \end{aligned}
% \end{equation}
% where ${\bar\alpha}_t  = \prod_{i=0}^{t}\alpha_i$ and $\nabla \log p_{\theta}(\bm{x}_t)$ indicates the the gradients of log likelihood with respect to $\bm{x}_t$ essentially describes what direction in data space to move in order to further increase its likelihood. Intuitively, since the $\epsilon_{\theta}(\bm{x}_t,t)$ predicts the noise added to $\bm{x}_t$, moving in its opposite direction, i.e., denoises the image, would be the best update to increase the subsequent log probability. 

% \textbf{Text-guided Diffusion Probabilistic Models.} Text-guided Diffusion Probabilistic Models aims to map a noise vector and textual condition $\mathcal{P}$ to an output image. The noise estimator $\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})$ is trained by~\myref{obj} while the term $\epsilon_{\theta}(\bm{x}_t, t)$ is substituted by $\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})$. Note that, $\mathcal{C} = \varphi(\mathcal{P})$ is the text embedding and $\varphi(\cdot)$ is a text encoder. It was found that 
% \begin{equation}\label{con_grdient}
%     \begin{aligned}
%         \epsilon_{\theta}(\bm{x}_t,t, \mathcal{C})=-\sqrt{1-\bar\alpha_t} \nabla \log p_{\theta}(\bm{x}_t | \mathcal{C})
%     \end{aligned}
% \end{equation}

% The DDIM sampling process corresponding to $\epsilon_{\theta}(\bm{x}_t,t, \mathcal{C})$ is defined as
% \begin{equation}\label{ddim2}
%     \begin{aligned}
%         {\bm{x}_{t-1}} = \sqrt{\frac{\alpha_{t-1}}{\alpha_t}}\bm{x}_t - \sqrt{\alpha_{t-1}}\psi(\alpha_t, \alpha_{t-1})\hat\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})
%     \end{aligned}
% \end{equation} 
% where $\hat\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})=\epsilon_{\theta}(\bm{x}_t, t, \emptyset) + \gamma \left[\epsilon_{\theta}(\bm{x}_t, t, \mathcal{C})-\epsilon_{\theta}(\bm{x}_t, \right.\\ \left. t, \emptyset )\right]$.
% $\epsilon_{\theta}(\bm{x}_t, t, \emptyset)$ is a unconditional DPM with null-text $\emptyset=\varphi(\text{``''})$, and $\gamma$ is a parameter that controls the strength of text guidance.


% % \begin{equation}
% %     \begin{aligned}
% %         \epsilon_{\theta}(\bm{x}_t, t, \mathcal{C}) = \min\limits_{\bm{\theta}} \mathbb{E}_{\bm{x}_0 \sim q(\bm{x}_0), \bm{\epsilon} \sim \mathcal{N}(\bm{0}, \bm{I}), t} \|\bm{\epsilon} - \epsilon_{\theta}(\bm{x}_t, t)\|_2^2 
% %     \end{aligned}
% % \end{equation}


% The noise estimator $\epsilon_{\theta}(\bm{x}_t, t)$



% Our


% is 

% added to
% a natural image to corrupt it, moving in its opposite direction "denoises" the image and would be the best
% update to increase the subsequent log probability. Our



% % \begin{equation}
% %     \begin{aligned}
% %         {\bm{x}_{t-1}} = \sqrt{\frac{\alpha_{t-1}}{\alpha_t}}\bm{x}_t - \sqrt{\alpha_{t-1}}\left(\sqrt{\frac{1}{\alpha_t}-1}-\sqrt{\frac{1}{\alpha_{t-1}}-1}\right)\epsilon_{\theta}(\bm{x}_t, t)
% %     \end{aligned}
% % \end{equation}



% % ~\ref{forward}. The resulting 
% % variable $\bm{x}_t$ can be formulated as:
% % \begin{equation}\label{forward}
% %   \begin{aligned}
% %       \bm{x}_t = \sqrt{\alpha_t}\bm{x}_0 + \sqrt{1-\alpha_t} \bm{\epsilon},   \quad \bm{\epsilon} \sim \mathcal{N}(0,1)
% %   \end{aligned}  
% % \end{equation}
% % where $\alpha_t = {\prod}_{s=1}^t(1-\beta_s)$, $\left\{{\beta}_s\right\}_{s=0}^T$ are fixed or learned variance schedule. 

% % Then, a neural network is trained to reverse that process, by minimizing the denoising objective, as shown in .
% % \begin{equation}
% %     \begin{aligned}
        
% %     \end{aligned}
% % \end{equation}



% a Gaussian transition $q(\bm{x}_{t} \mid \bm{x}_{t-1}) = \mathcal{N}(\sqrt{1- {\beta}_t}\bm{x}_{t-1}, {\beta}_t\bm{I})$, where $\left\{{\beta}_{t=0}^T\right\}$ are fixed or learned variance schedule. The resulting
% latent variable $\bm{x}_t$ can be formulated as:
% $$
% \bm{x}_t = \sqrt{\alpha_t}\bm{x}_0 + \sqrt{1-\alpha_t} \bm{\epsilon},   \quad \bm{\epsilon} \sim \mathcal{N}(0,1)
% $$

% where $\alpha_t = {\prod}_{s=1}^t(1-\beta_s)$.

% At reverse process, given a noise $\bm{x}_t$, the noise is gradually removed by another parametrized Gaussian transition $p_{\theta}(\bm{x}_{t-1} \mid \bm{x}_t) = \mathcal{N}(\bm{x}_{t-1};{\mu}_{\theta}(\bm{x}_t, t))$

% sequentially predicting it using our trained network for T steps.
% Since we aim



% αt := Q
% t
% s=1 (1 − βs).


% % Each step in the forward process is a Gaussian
% % transition q(xt | xt−1) := N (
% % √
% % 1 − βtxt−1, βtI), where
% % {βt}
% % T
% t=0 are fixed or learned variance schedule. The resulting
% latent variable xt can be expressed as:

% n that starts with z0, and gradually adds noise
% to obtain latent variables z1, z2, . . . , zT , following

% when sequentially sampling the latent variables


% denoising process that generates samples from Gaussian noise with a learnable model.


% trained to invert a diffusion process. For a number of timestep


% \textbf{Unconditional Denoising Diffusion Model.}

% \textbf{Text guidied diffusion model}

% \textbf{Denoising diffusion implicit models (DDIM).}



